Probing GNN Explainers: A Rigorous Theoretical and Empirical Analysis of GNN Explanation Methods

As Graph Neural Networks (GNNs) are increasingly being employed in critical real-world applications, several methods have been proposed in recent literature to explain the predictions of these models. However, there has been little to no work on systematically analyzing the reliability of these methods. Here, we introduce the first-ever theoretical analysis of the reliability of state-of-the-art GNN explanation methods. More specifically, we theoretically analyze the behavior of various state-of-the-art GNN explanation methods with respect to several desirable properties (e.g., faithfulness, stability, and fairness preservation) and establish upper bounds on the violation of these properties. We also empirically validate our theoretical results using extensive experimentation with nine real-world graph datasets. Our empirical results further shed light on several interesting insights about the behavior of state-of-the-art GNN explanation methods.

==> 020related_archive.tex <==
%This work encompasses explanation methods for Graph Neural Networks (GNNs) and their evaluation measures. Below we discuss the related work for each of these topics. \marinka{Lots of duplication. It needs revising and shortening.} 
% \hima{do we need some related work on generic explainability? dumping some below. can't copy this exactly but its fine to tweak a bit and use this.}
% \chirag{yes, I don't think we need an extensive discussion on them}
% Interpretability research can be categorized into learning inherently interpretable models, and constructing post hoc explanations. We provide an overview below. 
% \xhdr{Inherently Interpretable Models} Many approaches have been proposed to learn inherently interpretable models, for various tasks including classification and clustering. 
% To this end, various classes of models such as decision trees, decision lists~\cite{letham15:interpretable}, decision sets~\cite{lakkaraju16:interpretable}, prototype based models~\cite{bien2009classification, kim14:the-bayesian}, and generalized additive models~\cite{lou2012intelligible,caruana15:intelligible} were proposed. However, complex models such as deep neural networks often achieve higher accuracy than simpler  models~\cite{ribeiro2016should}; thus, there has been a lot of interest in constructing post hoc explanations to understand their behavior. 

% \chirag{push the related works to main tex but only include benchmarking and graphxai; and end it with the main contribution}
This paper builds upon a wealth of previous research at the intersection of \expmethods, graph neural networks and interpretability for graphs, and systematic evaluation of explanations. 

\xhdr{Post-hoc explanations and their analysis}
%
A myriad of techniques have been developed for explaining predictions in a post-hoc manner. These techniques 
differ in their access to the complex model (\ie black box vs. access to internals), scope of approximation (\ie global vs. local), search technique (\ie perturbation-based vs. gradient-based vs. surrogate-based), and basic units of explanation (\ie feature importance vs. rule based). In addition to LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified}, there are several other \emph{model-agnostic} \emph{local explanation} approaches that explain individual predictions~\cite{ribeiro2018anchors,slack2020i,koh2017understanding,simonyan2013saliency, sundararajan2017axiomatic, selvaraju2017grad,smilkov2017smoothgrad}.
%Several of these approaches rely on input perturbations to learn interpretable local approximations. 
%Other local explanation methods including SmoothGrad have been proposed to compute \emph{saliency maps} which capture local feature importance for an individual prediction by computing the gradient at that particular instance~\cite{simonyan2013saliency, sundararajan2017axiomatic, selvaraju2017grad,smilkov2017smoothgrad}. 
There has also been recent work on constructing \emph{counterfactual explanations} which capture what changes need to be made to an instance in order to flip its prediction~\citep{wachter2017counterfactual,ustun2019actionable,MACE,FACE,looveren2019interpretable, Barocas_2020, karimi2020algorithmic, karimi2020causal,agarwal2020explaining}, and \emph{global explanations} for summarizing the complete behavior of any given black box by approximating it using interpretable models~\citep{lakkaraju19faithful,bastani2017interpretability,kim2018interpretability}. 
%Such explanations can be leveraged to provide recourse to individuals negatively impacted by algorithmic decisions.
%An alternate approach is to construct \emph{global explanations} for summarizing the complete behavior of any given black box by approximating it using interpretable models~\cite{lakkaraju19:faithful,bastani2017interpretability,kim2018interpretability}. 

\looseness=-1
\xhdr{Explainability in Graph Neural Networks (GNNs)} 
%
%Graph neural networks are a prevailing learning paradigm for deep learning on graphs~\cite{li2021representation}. 
GNNs specify non-linear deep transformation functions that map graph structures (\ie nodes, edges or entire graphs) into compact vector embeddings~\citep{li2021representation}. This is typically achieved through a process that iteratively propagates neural messages along edges of a graph and aggregates them at nodes~\citep{gilmer2017neural}. A variety of GNN architectures have been proposed in the literature ~\citep{pareja2020evolvegcn,yun2019graph,zitnik2018modeling},
% that can embed diverse types of graphs, including temporal graphs~\cite{pareja2020evolvegcn}, knowledge graphs~\cite{yun2019graph}, and multi-relational graphs~\cite{zitnik2018modeling}
and recent research has focused on on developing GNN \expmethods~\citep{baldassarre2019explainability,faber2020contrastive,huang2020graphlime,lucic2021cf,luo2020parameterized,pope2019explainability,schlichtkrull2020interpreting,vu2020pgm,ying2019gnnexplainer}. Early methods developed graph analogs of \emph{gradient-based methods} from computer vision literature, including gradient heatmaps~\citep{Simonyan14a}, Grad-CAM~\citep{selvaraju2017grad}, and integrated gradients~\citep{sundararajan2017axiomatic}. More recently, \emph{perturbation-based methods} \citep{luo2020parameterized,schlichtkrull2020interpreting,ying2019gnnexplainer} explain GNN predictions by finding small subgraphs that are most influential for the prediction w.r.t. different perturbations of the input graph. 
To this end, GraphMASK~\citep{schlichtkrull2020interpreting} identifies edges in each GNN layer that can be dropped without affecting the final prediction. Similarly, GNNExplainer \citep{ying2019gnnexplainer} learns real-valued edge and node attribute masks that select influential subgraphs. Finally, \emph{surrogate-based methods} fit an interpretable model to local neighborhoods of target nodes such that the model faithfully represents GNN model's behavior in network vicinity of target nodes. For example, GraphLIME~\citep{huang2020graphlime} uses a feature-wise Hilbert-Schmidt independence criterion lasso (HSIC Lasso) as the surrogate model. %Here we provide the first answer to the question about which \expmethods have desirable properties for explaining GNN predictions and support our findings with theoretical analyses of all the above methods.

%Several approaches have been proposed to address the aforementioned challenge by explaining the predictions of GNNs. For instance, \textsc{GNNExplainer}~\cite{} is a model agnostic approach which takes a trained GNN and its predictions as inputs, and provides a compact subgraph and a small subset of node features as an explanation for each instance (e.g. a node or a graph). Each explanation is chosen such that it maximizes the mutual information with the corresponding GNN prediction. \textsc{PGExplainer}~\cite{} extends the above approach to achieve a global understanding of any learned GNN model. This approach adopts a deep neural network to parameterize the generation process of explanations, and thereby paves the way for naturally explaining multiple instances collectively. Furthermore, approaches such as \textsc{GraphLIME}~\cite{} leverage non-linear local approximations of GNNs to output node features crucial to predictions as explanations. Multiple gradient based approaches (e.g., vanilla gradients~\cite{} and integrated gradients~\cite{}) have also been used to explain individual predictions of GNNs. More recently, a post hoc approach called \textsc{GraphMask} proposes to interpret the predictions of GNNs by identifying unnecessary edges. This is done by learning a simple classifier for every edge which predicts if that edge can be dropped or not.

\looseness=-1
\xhdr{Evaluating explainers} 
%
% Recent work has shed light on the downsides of post-hoc explanation techniques.
% For instance, \cite{rudin2019stop} argued that post-hoc explanations unreliable as they are not necessarily faithful to the underlying models. % and can present spurious correlations.
% Further, empirical studies of explanations~\cite{adebayo2018sanity,slack2019can,lakkaraju2020how,rudin2019stop,dombrowski2019explanations, ghorbani2019interpretation} revealed several vulnerabilities of post-hoc explanations, including their fragility by demonstrating that explanations can change drastically when the input is perturbed~\cite{alvarez2018robustness}. 
% To this end, \cite{levine2019certifiably,pmlr-v119-chalasani20a,garreau2020looking} have made first steps towards analysing robustness and other properties of some post-hoc explanation techniques.
Few works have analysed robustness and other properties of post-hoc explanation techniques \citep{levine2019certifiably,pmlr-v119-chalasani20a,garreau2020looking}.
However, due to the relative infancy of GNN explainability as a field, rigorous analyses of GNN \expmethods are very limited; use a variety of qualitative and quantitative metrics for evaluating the correctness of explanations, including accuracy, faithfulness, and sparsity~\cite{sanchez2020evaluating,yuan2020explainability}; have been conducted only for specific cases; and theoretical analysis has not yet been attempted. As a result, these analyses are not necessarily generalizable and the issue gets further exacerbated as evaluation of \expmethods on real-world graph datasets is highly non-trivial due to the lack of ground-truth information. Further, qualitative evaluations can be subjective whereas quantitative evaluations are mostly driven by accuracy and do not consider other model properties.


% ROUGH
%However, due to the relative infancy of GNN explainability as a field, rigorous analyses of GNN \expmethods are very limited, have been conducted only for specific cases, and theoretical analysis has not yet been attempted. GNN \expmethods use a variety of qualitative and quantitative metrics for evaluating the correctness of explanations, including accuracy (how well an explanation matches ground-truth), faithfulness (how well the performance of an explanation matches model performance), and sparsity (how many node/edge attributes and edges are in an explanation)   ~\cite{sanchez2020evaluating,yuan2020explainability}. As a result, these analyses are not necessarily generalizable and the issue gets further exacerbated as evaluation of \expmethods on real-world graph datasets is highly non-trivial due to the lack of ground-truth information. Further, qualitative evaluations can be subjective whereas quantitative evaluations are mostly driven by accuracy and do not consider other model properties.
% Metrics:
% 1. talk about sparsity
% 2. accuracy
% 3. fidelity
% Problems:
% 1. qualitative are subjective
% 2. quantitative are mostly driven by accuracy and do not consider other model properties.
% 3. limited to attribution approaches with quantitative analysis
%\hima{some of these works e.g., ankur taly's integrated gradients and alvarez-millis's work talks about why stability is key; so we might need to spin the below text a bit more and/or move it to evaluating explainers piece.} 
% Recent studies have proposed several explanation methods to explain the predictions of GNNs \citep{baldassarre2019explainability,faber2020contrastive,huang2020graphlime,lucic2021cf,luo2020parameterized,pope2019explainability,schlichtkrull2020interpreting,vu2020pgm,ying2019gnnexplainer}. These methods can be broadly categorized into: a) gradient, b) perturbation, and (c) surrogate methods.
% Gradient-based graph explanation methods \citep{baldassarre2019explainability,pope2019explainability} are white-box approaches with complete access to the underlying model, including learned weights and intermediate node-embeddings.
% Perturbation-based methods \citep{luo2020parameterized,schlichtkrull2020interpreting,ying2019gnnexplainer} are model-agnostic black-box approaches, \ie they treat the GNN as an oracle (black-box) and only use the model's output for generating explanations. Perturbation methods perturb the input graph and use the resulting prediction changes to produce explanations.
% While the idea is principle in causal reasoning, the
% physical interventions---taking a node/edge out of a graph while keeping the rest unchanged---is impractical in most real-world graphs.
% Surrogate methods \citep{huang2020graphlime,vu2020pgm} sample a dataset using the local neighborhood of a given node and then fit an interpretable model to the sampled dataset. Finally, they use the explanations of the interpretable model as an explanation for the node predictions of the GNN model.
\hide{
\Expmethods for GNNs can be broadly categorized into: a) gradient-, b) perturbation-, and (c) surrogate-based methods. Here we briefly describe some of the methods we theoretically analyze in Sec.~\ref{sec:theory}. See Sec.~\ref{app:sec_exp_methods} for an in-depth overview of these methods.
Gradient-based graph explanation methods \citep{baldassarre2019explainability,pope2019explainability} are white-box approaches with complete access to the underlying model, including learned weights and intermediate node-embeddings.
Vanilla gradient methods leverage the gradient of a model $f$ with respect to the node attributes $\mathbf{x}_{u}$: $\triangledown_{\mathbf{x}_{u}}f$ to indicate the importance of different input attributes.

Perturbation-based methods \citep{luo2020parameterized,schlichtkrull2020interpreting,ying2019gnnexplainer} are model-agnostic black-box approaches, \ie they treat the GNN as an oracle (black-box) and only use the model's output for generating explanations. These methods perturb the input graph and use the resulting prediction changes as explanations.
% While the idea is principle in causal reasoning, the physical interventions---taking a node/edge out of a graph while keeping the rest unchanged---is impractical in most real-world graphs.
% Perturbation-based methods \citep{luo2020parameterized,schlichtkrull2020interpreting,ying2019gnnexplainer} quantifies the change of a model's output predictions with respect to different input perturbations. 
For perturbation-bases methods, we analyze GraphMASK \citep{schlichtkrull2020interpreting} that identifies edges in individual model layers that can be dropped without affecting the output model predictions. It learns a binary choice $z^{l}_{u, v}$ that indicates whether an edge connecting node $u$ and $v$ in layer $l$ can be dropped, and then replaces it with a learned baseline.
GraphMASK learns $z^{l}_{u,v}$ for all $(u,v) \in \mathcal{E}$ for the training data points using an erasure function.
For explaining a given prediction, GraphMASK uses the trained erasure function to generate masked representations of the graph.
% using: $\Tilde{h}_{u}^{l}{=} \mathbf{Z}^{l}\circ h_{u}^{l} + \alpha^{l}\circ(1-\mathbf{Z}^{l})$, where $\mathbf{Z}^{l}$ comprises of all the individual binary scores $z^{l}_{u, v}=g_{\pi}(h_{u}^{l}, h_{v}^{l})$, $\alpha^{l}$ is the learned baseline, and `$\circ$' denotes the element-wise Hadamard product.

Finally, surrogate-based methods provide instance-level explanations by employing an interpretable surrogate model to approximate the predictions of complex non-linear GNNs for a small sampled dataset around an input node. Finally, they use the explanations of the interpretable model as an explanation for the node predictions of the GNN model. Here, we investigate GraphLIME \citep{huang2020graphlime} which is a local interpretable model explanation for GNNs that identifies a nonlinear interpretable model over the neighbors of a node that is locally faithful to the node's prediction.
It considers a node attribute-wise kernelized nonlinear method called Hilbert-Schmidt Independence Criterion Lasso (HSIC Lasso) as an explanation model.

where preliminary approaches developed graph analogs of gradient-based methods like gradient heatmaps \citep{Simonyan14a}, Grad-CAM \citep{selvaraju2017grad}, and integrated gradients \citep{sundararajan2017axiomatic} from computer vision literature. These methods are model-dependent and need access to the underlying GNN model. To mitigate this, other popular approaches include perturbation-based \citep{ying2019gnnexplainer,schlichtkrull2020interpreting} and surrogate-based \citep{huang2020graphlime,vu2020pgm} methods. To this end, GNNExplainer \citep{ying2019gnnexplainer} proposed a model-agnostic \expmethod that learns a real-valued mask graph mask which selects an important subgraph of the GNN's computational graph. More recently, GraphMASK \citep{schlichtkrull2020interpreting} presented an approach that learns an erasure function for predicting whether an edge connection should be retained.
Furthermore, methods like GraphLIME \citep{huang2020graphlime} learn interpretable models using nodes' N-hop neighborhood and then outputs the most representative attributes as the explanations of the GNN prediction.
}

==> 040theory.tex <==
% \chirag{Editing here}
% \hima{Let's do all unfaithfulness, all group unfairness, all counterfactual unfairness, and all instability in separate subsections. Move all descriptions of methods from 4.3 and 4.4 to preliminaries. We would anyways need to add short descriptions of each of the methods we talk about in preliminaries. We can just say \\
% 4. Theoretical Analysis;  \\
% 4.1 Analyzing the Faithfulness of GNN \expmethods; \\
% 4.2 Analyzing the Fairness of GNN \expmethods;\\
% 4.2.1 group fairness, 4.2.2 counterfactual fairness; \\
% 4.3 Analyzing the Stability of GNN \expmethods.
% }
\chirag{Hima!}Next, we derive theoretical bounds for faithfulness (Sec.~\ref{sec:unfaithfulness-theory}), stability (Sec.~\ref{sec:instability-theory}), and fairness (Sec.~\ref{sec:unfairness-theory}) for GNN \expmethods. These bounds only need information about a GNN's message passing form~\cite{gilmer2017neural} and do not make any assumptions about it's architecture. As we will show, our bounds apply to all commonly used \expmethods and can be computed efficiently, making them suitable for use in empirically evaluating the reliability of explanations.
% output by an \expmethod.
% Next we derive theoretical bounds of faithfulness (Sec.~\ref{sec:unfaithfulness-theory}), stability (Sec.~\ref{sec:instability-theory}), and fairness (Sec.~\ref{sec:unfairness-theory}) for GNN \expmethods. These bounds only need information about the message passing form of GNNs~\cite{gilmer2017neural} and do not make any assumptions about their architecture. As we will show, the proposed bounds apply to all commonly used GNN \expmethods and can be computed efficiently, which makes them suitable for use in empirical evaluations and for analyzing the reliability of explanations output by an \expmethod.
% when one wishes to find out which of several \expmethods produces most reliable explanations.
%Note, the bounds for faithfulness and group fairness encompass the entire range of GNN \expmethods that generate explanations using node features or edges.
% and local-group unfairness of all \expmethods that generate explanations in the node-feature or graph-structure level (Sec.~\ref{sec:local_group_faith}). This unified framework encompass the entire range of GNN \expmethods and aids in analyzing their faithful and fairness properties.
% We then select one representative method from perturbation- (Sec.~\ref{sec:graphlime}), gradient- (Sec.~\ref{sec:gradient}), and surrogate-based (Sec.~\ref{sec:graphmask}) methods and derive upper bounds for stability and counterfactual fairness.

\subsection{Analyzing Faithfulness of GNN Explanation Methods}\label{sec:unfaithfulness-theory}
Here, we derive upper bounds on unfaithfulness of explanations output by GNN \expmethods.

\xhdr{Theorem 1} \textit{Given a node $u$ and a set $\mathcal{K}$ of node perturbations, the faithfulness property (Sec.~\ref{sec:def_faith}, Eqn.~\ref{eq:faith}) of its explanation $E_{u}$ can be bounded as follows:}
\begin{equation}
    \sum_{u'\in\mathcal{K}}||f(\mathcal{G}_{u'}) - f(t(E_{u}, \mathcal{G}_{u'})) ||_{2} \leq \gamma~(1 + |\mathcal{K}|)~||\Delta||_{2},
    \label{eq:unfaithful}
\end{equation}
where $f(\mathcal{G}_{u'}) =\mathbf{\hat{y}}_{u'}$ are softmax predictions that use original attributes and $f(t(E_{u}, \mathcal{G}_{u'}))=\mathbf{\hat{y}}_{u'}^{E}$ are softmax predictions that use attributes marked important by explanation $E_{u}$. Further, $\gamma$ denotes the product of the Lipschitz constants for GNN's activation function and GNN's weight matrices across all layers in the GNN, and $\Delta$ is an \expmethod-specific term.

\textit{Proof Sketch.~} We show that faithfulness of an \expmethod, which generates node attribute explanations, is bounded by $\gamma_{11}~(1{+}|\mathcal{K}|)~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u}||_{2}$, where $\gamma_{11}$ is a constant comprising of the product of the Lipschitz constant for GNN's activation function, weights of the final node classification layer, and self-attention weight of node $u$ across all layers of the GNN.
Further, we show that faithfulness of an \expmethod, which generates edge-level explanations, is bounded by $\gamma_{12}~(1{+}|\mathcal{K}|)~||\Delta_{\mathbf{x}_{v}}||_{2}$, where $\gamma_{12}$ is similar to $\gamma_{11}$ but uses weights associated with $u$'s immediate neighbors instead of self-attention weight, and $\Delta_{\mathbf{x}_{v}}$ is the difference between embeddings of $u$'s neighbors where we exclude edges that are not part of the explanation (\ie unnecessary edges as identified by the explanation). Details are in Appendix~\ref{app:local_group_faith}.
% Without loss of generality, we use a two-layer GNN model for our proof and show how the proof extends to a GNN model with $L$ layers. The two-layer model is defined as:
% \begin{align*}
%     % & \hat{y}_{u}{=}\text{softmax}(\mathbf{h}_{u}^{2})\\
%     & \mathbf{h}_{u}^{1}{=}\text{sp}(\mathbf{W}_{a}^{1}\mathbf{x}_{u}+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}}\mathbf{x}_{v}) \\
%     & \mathbf{h}_{u}^{2}{=}\mathbf{W}_{\text{fc}}\mathbf{h}_{u}^{1}+\mathbf{b}\\
%     & \mathbf{\hat{y}}_{u}{=}\text{softmax}(\mathbf{h}_{u}^{2}),
% \end{align*}
% where $\mathbf{W}_{n}^{1}$ is the weight matrix associated with the neighbors of node $u$, $\mathbf{W}_{a}^{1}$ is the self-attention weight matrix at layer one, and ``sp'' is the softplus activation function.
% For the fully-connected layer, we have $\mathbf{W}_{\text{fc}}$ as the weight matrix and $\mathbf{b}$ as the bias term.
% The softplus function is a smooth approximation of the ReLU function.
% We generate $|\mathcal{K}|$ perturbations of node $u$ by adding normal Gaussian noise to the node features, \ie $\mathbf{x}_{u'}{=}\mathbf{x}_{u}{+}\tau$, and rewire edges with some probability $p_{r}$.
% For faithfulness, we get the predictions for node $u$ using the weighted node features of node $u$, \ie the element-wise product between $\mathbf{r}_{u}$ (the feature importance mask generated as an explanation) and $\mathbf{x}_{u}$. Let $\mathbf{\hat{y}}_{u}^{E}$ denote the softmax output for node $u$ using the explanation $E_{u}$, \ie $f(t(E_{u}, \mathcal{G}_{u}))$. Therefore, the updated equations using the explanations are:
% % Therefore, $\mathbf{h}_{u}^{1'} = \text{softplus}(\mathbf{W}_{a}^{1}\mathbf{x}_{u}^{'}+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v})$.
% \begin{align*}
%     & (\mathbf{h}_{u}^{1})^{E}=\text{sp}\big(\mathbf{W}_{a}^{1}(\mathbf{r}_{u}\circ\mathbf{x}_{u})+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v}\big)\\
%     & (\mathbf{h}_{u}^{2})^{E}=\mathbf{W}_{\text{fc}}(\mathbf{h}_{u}^{1})^{E}+\mathbf{b}\\
%     & \mathbf{\hat{y}}_{u}^{E}=\text{softmax}((\mathbf{h}_{u}^{2})^{E}),
% \end{align*}
% where $\mathcal{N}'_{u}$ denotes the new neighborhood for node $u$ due to the adjacency mask matrix $\mathbf{R}_{u}$.
% The difference between the predicted labels for the original and the important node features can be given as:
% \begin{equation}
%     \mathbf{\hat{y}}_{u} - \mathbf{\hat{y}}_{u}^{E} = \text{softmax}(\mathbf{h}_{u}^{2})-\text{softmax}((\mathbf{h}_{u}^{2})^{E})
%     \label{eq:faith_1}
% \end{equation}

% \xhdr{Corollary 1} \textit{For any differentiable function $g: \mathbb{R}^{a} \to \mathbb{R}^{b}$,}
% \begin{equation}
%     || g(x) - g(y) ||_{2} \leq ||\mathbf{J}||^{*}_{F}||x-y||_{2}~~~~ \forall x, y \in \mathbb{R},
% \end{equation}
% where $||\mathbf{J}||^{*}_{F} = \max_{x} ||\mathbf{J}||_{F}$ and $\mathbf{J}$ is the Jacobian matrix of $g(x)$ w.r.t. $x$. This is implied from the mean value theorem, where for any function $g(x)$ and its derivative $\deriv{g(x)}{x}$, we have: $g(x) - g(y)=\deriv{g(\phi)}{\phi}(x-y)$, for some $\phi \in (y, x)$.
% Hence, taking the norm on both sides in Eqn.~\ref{eq:faith_1}, we get,
% \begin{align*}
%     & ||\mathbf{\hat{y}}_{u} - \mathbf{\hat{y}}_{u}^{E}||_{2} = ||\text{softmax}(\mathbf{h}_{u}^{2})-\text{softmax}((\mathbf{h}_{u}^{2})^{E})||_{2}\\
%     & \leq \mathcal{C}_{\text{fc}}||\mathbf{h}_{u}^{2}-(\mathbf{h}_{u}^{2})^{E}||_{2} \tag{Using Corollary 1},\\
% \end{align*}
% where $\mathcal{C}_{\text{fc}}$ represents the Lipschitz constant for the softmax function.
% Substituting the values of $\mathbf{h}_{u}^{2}$ and $(\mathbf{h}_{u}^{2})^{E}$ we get:
% \begin{align*}
%     & ||\mathbf{\hat{y}}_{u} - \mathbf{\hat{y}}_{u}^{E}||_{2} \leq 
%     \mathcal{C}_{\text{fc}}||\mathbf{W}_{\text{fc}}\mathbf{h}_{u}^{1}+\mathbf{b} -\mathbf{W}_{\text{fc}}(\mathbf{h}_{u}^{1})^{E}-\mathbf{b}||_{2} \\
%     & \leq 
%     \mathcal{C}_{\text{fc}}||\mathbf{W}_{\text{fc}}\mathbf{h}_{u}^{1}-\mathbf{W}_{\text{fc}}(\mathbf{h}_{u}^{1})^{E}||_{2} \\
%     & \leq 
%     \mathcal{C}_{\text{fc}}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{h}_{u}^{1} -(\mathbf{h}_{u}^{1})^{E}||_{2} \tag{Using Cauchy-Schwartz inequality} \\
% \end{align*}
% Substituting the values of $\mathbf{h}_{u}^{1}$ and $(\mathbf{h}_{u}^{1})^{E}$ we get:
% \begin{align*}
%     & ||\mathbf{\hat{y}}_{u} - \mathbf{\hat{y}}_{u}^{E}||_{2} \leq 
%     \mathcal{C}_{\text{fc}}~||\mathbf{W}_{\text{fc}}||_{2}~||\text{sp}\big(\mathbf{W}_{a}^{1}\mathbf{x}_{u}+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v}\big) - \text{sp}\big(\mathbf{W}_{a}^{1}(\mathbf{r}_{u}\circ\mathbf{x}_{u})+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v}\big)||_{2} \\
%     & \leq 
%     \mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{W}_{a}^{1}\mathbf{x}_{u}+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v} - \mathbf{W}_{a}^{1}(\mathbf{r}_{u}\circ\mathbf{x}_{u})-\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v}||_{2} \tag{Using Corollary 1}\\
%     & \leq 
%     \mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~\big(||\mathbf{W}_{a}^{1}\big(\mathbf{x}_{u} - (\mathbf{r}_{u}\circ\mathbf{x}_{u})\big)||_{2} + ||\mathbf{W}_{n}^{1}\Delta_{\mathbf{x}_{v}}||_{2}\big), \tag{Using triangle inequality}
%     % & \leq \mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{W}_{a}^{1}||_{2}~||\mathbf{x}_{u} - (\mathbf{r}_{u}\circ\mathbf{x}_{u})||_{2} \tag{Using Cauchy-Schwartz inequality}
% \end{align*}
% where $\Delta_{\mathbf{x}_{v}}$ is the difference between the representations of the neighbors of $u$ after dropping edges using the edge masks. This difference can be neglected for gradient and GraphLIME methods as they provide explanations in the node feature space. 
% % and  the  and is assumed to be very small because the model is smooth function and large restructuring of the graph can lead to different representations for the node \cite{schlichtkrull2020interpreting}. 
% Now, using Cauchy-Schwartz inequality, the prediction difference for a node $u$ using its original and just important node features is bounded by:
% \begin{equation}
%     ||\mathbf{\hat{y}}_{u} - \mathbf{\hat{y}}_{u}^{E}||_{2} \leq \mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{W}_{a}^{1}||_{2}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u})||_{2},
%     \label{eq:faith_2}
% \end{equation}
% where $\mathcal{C}_{1}$ is the Lipschitz constant for the softplus activation function and $\mathbf{1} \in \mathbb{R}^{M}$ is vector with all ones. For mathematical brevity, let $\gamma_{11}=\mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{W}_{a}^{1}||_{2}$. Similarly, the prediction difference for GraphMASK which provides an explanation with respect to edges is bounded by:
% \begin{equation}
%     ||\mathbf{\hat{y}}_{u} - \mathbf{\hat{y}}_{u}^{E}||_{2} \leq 
%     \mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{W}_{n}^{1}||_{2}~||\Delta_{\mathbf{x}_{v}}||_{2},
%     \label{eq:faith_edge}
% \end{equation}
% where $\gamma_{12}=\mathcal{C}_{\text{fc}}~\mathcal{C}_{1}~||\mathbf{W}_{\text{fc}}||_{2}~||\mathbf{W}_{n}^{1}||_{2}$.
% \xhdr{Node feature explanations} Since all the perturbed nodes use the same node feature explanation $\mathbf{r}_{u}$, 
% % the probability $p_{r}$ of rewiring an edge is very small to maintain the underlying graph structure, 
% we obtain the difference between the predictions for a perturbed node $k$  using the perturbed and the masked node features, \ie
% \begin{align*}
%     & ||\mathbf{\hat{y}}_{k}^{'} - \mathbf{\hat{y}}_{k}^{E}||_{2} \leq
%     \gamma_{11}~||\mathbf{x}_{k'} - (\mathbf{r}_{u}\circ\mathbf{x}_{k'})||_{2},
% \end{align*}
% where $\mathbf{\hat{y}}_{k}^{'}$ is the softmax prediction using the perturbed node feature $\mathbf{x}_{k'}=\mathbf{x}_{u}+\tau$, and as per the definition of local-group faithfulness we use the explanation mask of node $u$ for node $k$. Finally, we get:
% \begin{equation}
%     ||\mathbf{\hat{y}}_{k}^{'} - \mathbf{\hat{y}}_{k}^{E}||_{2} \leq 
%     \gamma_{11}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{k'}||_{2}
%     \label{eq:faith_3}
% \end{equation}
% For local-group faithfulness, we generate a set of $\mathcal{K}$ perturbed nodes and get $|\mathcal{K}|$ predictions from the model for each of the corresponding perturbations. Using Eqns.~\ref{eq:faith_2} and \ref{eq:faith_3}, and getting the predictions from all $|\mathcal{K}|$ perturbations, we get:
% \begin{align*}
%     % & ||\hat{y}_{u} - \hat{y}_{u}^{E}||_{2} + \sum_{k{=}1}^{\mathcal{K}}||\hat{y}_{k}^{'} - \hat{y}_{k}^{E}||_{2} \leq \gamma_{1}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u})||_{2} + \gamma_{1}\sum_{k{=}1}^{\mathcal{K}}~||(\mathbf{1}-\mathbf{r}_{u})\circ(\mathbf{x}_{u}^{'})_{k}||_{2}\\
%     & \sum_{u'\in\mathcal{K}}||\mathbf{\hat{y}}_{u'} - \mathbf{\hat{y}}_{u'}^{E}||_{2} \leq \gamma_{11}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u})||_{2} + \gamma_{11}\sum_{u'\in \mathcal{K}}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u'}||_{2}\\
%     & \leq \gamma_{11}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u})||_{2} + \gamma_{11}~||(\mathbf{1}-\mathbf{r}_{u})\circ\sum_{u'\in \mathcal{K}}\mathbf{x}_{u'}||_{2},
% \end{align*}
% where $\mathbf{\hat{y}}_{u'}$ represents the softmax prediction of node $u'$.
% % $(\mathbf{x}_{u}^{'})_{k}$ and $k \in \{1\dots\mathcal{K}\}$. 
% Assuming $\tau$ to be drawn from a normal distribution, we get:
% $\sum_{u'\in \mathcal{K}}\mathbf{x}_{u'} = |\mathcal{K}|\mathbf{x}_{u} + \sum_{u'\in \mathcal{K}}\tau_{k}$. For sufficiently large $|\mathcal{K}|$, we have: $\sum_{u'\in \mathcal{K}}(\mathbf{x}_{u}^{'})_{k} \approx |\mathcal{K}|\mathbf{x}_{u}$.
% Putting everything together, 
% \begin{align*}
%     & \sum_{u'\in\mathcal{K}}||\mathbf{\hat{y}}_{u'} - \mathbf{\hat{y}}_{u'}^{E}||_{2} \leq \gamma_{11}~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u})||_{2} + \gamma_{11}~|\mathcal{K}|~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u}||_{2}\\
%     & \leq \gamma_{11}~(1 + |\mathcal{K}|)~||(\mathbf{1}-\mathbf{r}_{u})\circ\mathbf{x}_{u}||_{2}
% \end{align*}
% % the term on the left-side of the inequality represents the local-group faithfulness w.r.t. a single explanation for node $u$ (as defined in Eqn.~\ref{eq:faith}).
% For a GNN model with $L$ message-passing layers and one fully-connected layer for node classification, $\gamma_{11}$ takes the general form of:
% \begin{equation}
%     \gamma_{11} = \mathcal{C}_{\text{fc}}~||\mathbf{W}_{\text{fc}}||_{2}~\prod_{l=1}^{L}\mathcal{C}_{l}||\mathbf{W}_{a}^{l}||_{2},
%     \label{eq:gamma_all}
% \end{equation}
% where $\mathcal{C}_{\text{fc}}$ is the Lipschitz constant for the softmax activation operating on the fully-connected layer, $\mathbf{W}_{\text{fc}}$ is the weight matrix associated with the fully-connected layer, $\mathcal{C}_{l}$ is the Lipschitz constant of the softplus activation of each message-passing layer, and $\mathbf{W}_{a}^{l}$ is the self-attention weight associated with the $l$-th message-passing layer.
% \xhdr{Edge explanations} Note, the difference between the predictions for a perturbed node $k$ using the perturbed and the masked node features will be similar to Eqn.~\ref{eq:faith_edge} as for local-group faithfulness, the perturbations are made only in node $u$, \ie
% \begin{align*}
%     ||\mathbf{\hat{y}}_{k}^{'} - \mathbf{\hat{y}}_{k}^{E}||_{2} \leq 
%     \gamma_{12}~||\Delta_{\mathbf{x}_{v}}||_{2},
%     \label{eq:faith_edge}
% \end{align*}
% Also, since we use the same explanation for all the nodes in set $\mathcal{K}$, the bound for local-group faithfulness using edge explanations is given by:
% \begin{align*}
%     & \sum_{u'\in\mathcal{K}}||\mathbf{\hat{y}}_{u'} - \mathbf{\hat{y}}_{u'}^{E}||_{2} \leq \gamma_{12}~(1 + |\mathcal{K}|)~||\Delta_{\mathbf{x}_{v}}||_{2},
% \end{align*}
% where as in Eqn.~\ref{eq:gamma_all}, $\gamma_{12}$ can take the general form for $L$ message-passing layers as: $\gamma_{12} = \mathcal{C}_{\text{fc}}~||\mathbf{W}_{\text{fc}}||_{2}~\prod_{l=1}^{L}\mathcal{C}_{l}||\mathbf{W}_{n}^{l}||_{2}$.
\subsection{Analyzing Stability of GNN Explanation Methods} \label{sec:instability-theory}
Next, we take a representative \expmethod for each of gradient- (Gradients \cite{Simonyan14a}), perturbation- (GraphMASK \cite{schlichtkrull2020interpreting}), and surrogate-based (GraphLIME \cite{huang2020graphlime}) methods and derive upper bounds on the stability of their explanations.

% \subsubsection{Gradient method: GNN Gradients}
% \label{sec:instability-grad}
\xhdr{Theorem 2 (Gradients)} \textit{Given a non-linear activation function $\sigma$ that is Lipschitz continuous, the stability property (Sec.~\ref{sec:def_stable}, Eqn.~\ref{eq:stable}) of explanation $E_{u}$ returned by Gradients method can be bounded as follows:}
% explanation $E_u$ returned by the Gradients method is stable, \ie}
% \vspace*{-\abovedisplayskip}
\begin{equation}
    ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq \gamma_{3}||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p},
    \label{eq:grad_stable}
\end{equation}
% \vskip -0.1in
where $\gamma_{3}$ is a constant, $\mathbf{x}_{u}$ is $u$'s attribute vector, and $\mathbf{x}_{u'}$ is the perturbed attribute vector.

\textit{Proof Sketch.~} We prove that gradient explanations are Lipschitz using data processing inequalities and the Lipschitz constant ($\gamma_{3}$) is the product of the $\ell_{\text{p}}$-norm of the difference in the predictions between the original and perturbed node, the weight of the final classification layer, and the weights associated with node $u$. Details are in Appendix~\ref{app:gradient_instability}.
% Similar to Sec.~\ref{sec:local_group_faith}, let us consider a two-layer GNN model trained on a node classification task using softmax cross-entropy loss function with the first layer a message-passing GNN layer and the second layer as a fully-connected layer. The cross-entropy (CE) loss is given as:
% \begin{equation}
%     \text{CE} = -\sum_{i} y_{i}\log \hat{y}_{u},  % \hat{y}_{i},
% \end{equation}
% where $\mathbf{y}$ is a vector with one one non-zero element (which is 1), $\mathbf{\hat{y}}_{u}{=}\text{softmax}(\mathbf{h}_{u}^{2})$, $\mathbf{h}_{u}^{2}{=}\mathbf{W}_{\text{fc}}\mathbf{h}_{u}^{1} + \mathbf{b}$, and $\mathbf{h}_{u}^{1}{=}\text{sp}(\mathbf{W}_{a}^{1}\mathbf{x}_{u} + \mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v})$.
% $\mathbf{W}_{n}^{1}$ is the weight matrix associated with the neighbors of node $u$ and $\mathbf{W}_{a}^{1}$ is the self-attention weight matrix at layer one.
% For the fully-connected layer, we have $\mathbf{W}_{\text{fc}}$ as the weight matrix and $\mathbf{b}$ as the bias term.
% ``sp'' is the softplus activation function which is a smooth approximation of the ReLU function.
% For stability, we generate $\mathbf{x}_{u'}$ by adding noise to the node features of node $u$ and keep everything else constant. Therefore, $\mathbf{h}_{u'}^{1} = \text{sp}(\mathbf{W}_{a}^{1}\mathbf{x}_{u'}+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v})$.
% Now, the differentiation of the model \textit{w.r.t.} the node features can be given as:
% \begin{align*}
%     \triangledown_{\mathbf{x}_{u}}f = \deriv{(\text{CE})}{\mathbf{x}_{u}} = \deriv{(\text{CE})}{\mathbf{h}_{u}^{2}}\deriv{\mathbf{h}_{u}^{2}}{\mathbf{h}_{u}^{1}}\deriv{\mathbf{h}_{u}^{1}}{\mathbf{x}_{u}}, \tag{By chain rule}
% \end{align*}
% Note, the advantage of using \textit{softplus} activation function is that it is differentiable for all $x$, \ie
% \begin{align*}
%     & \text{sp}(x)=\textit{ln}(1+\exp^{x}) \\
%     & \deriv{(\text{sp}(x))}{\text{x}} = \frac{\exp^{x}}{1 + \exp^{x}} \cdot \frac{(1/\exp^{x})}{(1/\exp^{x})}\\
%     & = \frac{1}{1 + \exp^{-x}}\\
%     & = \sigma(x),
% \end{align*}
% where $\sigma(\cdot)$ is the sigmoid activation function. Putting it all together we get,
% \begin{eqnarray}
%     \triangledown_{\mathbf{x}_{u}}f = (\mathbf{y}_{u}-\mathbf{\hat{y}}_{u})(\mathbf{W}_{\text{fc}})^{T}\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u} + \mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v})(\mathbf{W}_{a}^{1})^{T}\\
%     \triangledown_{\mathbf{x}_{u'}}f = (\mathbf{y}_{u}-\mathbf{\hat{y}}_{u})(\mathbf{W}_{\text{fc}})^{T}\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u'} + \mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v})(\mathbf{W}_{a}^{1})^{T}
% \end{eqnarray}
% Note, $\mathbf{\hat{y}}_{u}$ is same for both  original and perturbed node according to the Definition 2 in Sec.~\ref{sec:problem} and we drop the second neighborhood term since the probability ($p_{r}$) of rewiring the edges is very small to maintain the original graph structure.
% Hence, subtracting the explanations (model gradients) for the original and perturbed node features and taking the norm on both sides, we get:
% \begin{align*}
%     & ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} = ||(\mathbf{y}_{u}-\mathbf{\hat{y}}_{u})(\mathbf{W}_{\text{fc}})^{T}\big(\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u'})-\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u})\big)(\mathbf{W}_{a}^{1})^{T}||_{p},\\
% \end{align*}
% Using Cauchy-Schwartz inequality, we get:
% \begin{align*}
%     & ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u'})-\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u})||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}
% \end{align*}
% Assuming that $\sigma(\cdot)$ is normalized Lipschitz, \ie $||\sigma{(b)}-\sigma{(a)}||_{p} \leq ||b-a||_{p}$, we get,
% \begin{align*}
%     & ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}\mathbf{x}_{u'}-\mathbf{W}_{a}^{1}\mathbf{x}_{u}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}\\
%     & \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}(\mathbf{x}_{u'}-\mathbf{x}_{u})||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}\\
%     & \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}||_{p}~||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p} \tag{Using Cauchy-Schwartz inequality}\\
%     & \leq \gamma_{3}~||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p},
% \end{align*}
% where $\gamma_{3} = ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}$.
% For a GNN model with $L$ message-passing layers and one fully-connected layer for node classification, $\gamma_{3}$ takes the general form of:
% \begin{equation}
%     \gamma_{3} = ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~\prod_{l=1}^{L}||\mathbf{W}_{a}^{l}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p},
%     % \mathcal{C}_{\text{fc}}~||\mathbf{W}_{\text{fc}}||_{2}~\prod_{l=1}^{L}\mathcal{C}_{l}||\mathbf{W}_{a}^{l}||_{2},
% \end{equation}
% where $\mathbf{W}_{a}^{l}$ is the self-attention weight associated with the $l$-th message-passing layer.

% \subsubsection{Perturbation method: GraphMASK}
% \label{sec:instability-graphmask}
\xhdr{Theorem 3 (GraphMASK)} \textit{Given concatenated embeddings of node $u$ and $v$, the stability property (Sec.~\ref{sec:def_stable}, Eqn.~\ref{eq:stable}) of explanation $E_{u}$ returned by GraphMASK method can be bounded as follows:}
% explanation $E_{u}$ returned by the GraphMASK method for layer $l$ is stable, \ie}
% \vspace*{-\abovedisplayskip}
\begin{equation}
    ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq \gamma_{4}^{l}~||\mathbf{q}^{l}_{u',v} - \mathbf{q}^{l}_{u,v}||_{2},
    \label{eq:gmask_stable}
\end{equation}
where $E_{u}$ is an edge mask comprising of $z^{l}_{u, v}$ indicating whether an edge connecting node $u$ and $v$ in layer $l$ can be dropped or not, $q^{l}_{u,v}$ is the concatenated embeddings for node $u$ and $v$ at layer $l$, and $\gamma_{4}^{l}$ denotes the Lipschitz constant which is a product of the weights of the $l$-th fully-connected layer, and the Lipschitz constants for the layer normalization function and softplus activation function.

\textit{Proof Sketch.} We prove that a GraphMASK's explanation for an edge at layer $l$ is Lipschitz continuous and the Lipschitz constant ($\gamma_{4}^{l}$) is product of the Lipschitz constants of the layer's normalization function and the $\ell_{2}$-norm of the weight matrices of the erasure function. Details are in Appendix~\ref{app:graphmask_instability}.

% \subsubsection{Surrogate method: GraphLIME}
% \label{sec:instability-graphlime}
\xhdr{Theorem 4 (GraphLIME)} \textit{Given the centered Gram matrices for the original and perturbed node attributes, the stability property (Sec.~\ref{sec:def_stable}, Eqn.~\ref{eq:stable}) of explanation $E_{u}$ returned by GraphLIME method can be bounded as follows:}
% explanation $E_{u}$ returned by the GraphLIME method for the $k$-th node feature is stable, \ie}
% \vspace*{-\abovedisplayskip}
\begin{equation}
    ||\beta^{'}_{k} - \beta_{k}||_{F} \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
    % ||\text{GLIME}(\mathbf{K}^{(k)^{'}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
\end{equation}
% \vskip -0.1in
where $E_{u}$ is a node mask produced using the attribute importance $\beta^{'}_{k}$ and $\beta_{k}$ generated by GraphLIME for the % the $\mathbf{K}^{(k)}$ and $\mathbf{K}^{(k)^{'}}$ are the centered Gram matrix 
perturbed and original node attributes, $\gamma_{2}$ is a constant independent of the added noise, $\mathbf{e}$ is a vector of all ones, and $\mathbf{W}$ is a matrix comprising of the added noise terms.

\textit{Proof Sketch.~} We prove that the stability of GraphLIME is bounded by the trace of the Gram matrix for the output label and of the perturbed Gram matrix due to the noise added in the input graph. We first derive the closed-form of the attribute importance coefficient $\beta$ and then use it derive the upper bounds for the GraphLIMEs' stability. Details are in Appendix~\ref{app:graphlime_instability}.

\subsection{Analyzing Fairness of GNN Explanation Methods} \label{sec:unfairness-theory}
Here, we analyze the group fairness (Sec.~\ref{sec:lg-unfairness-theory}) and counterfactual fairness (Sec.~\ref{sec:counter-unfairness-theory}) properties of state-of-the-art GNN \expmethods and derive their corresponding bounds.
\subsubsection{Group Fairness}
\label{sec:lg-unfairness-theory}
Here, we provide a bound on how well the explanations output by GNN explainers preserve group fairness.
%A model satisfies group fairness if the instances in the protected and unprotected groups have equal probability of being assigned to the positive predicted class. In this context, the unfairness property is dependent on the faithfulness of an \expmethod, \ie the group unfairness of node $u$ for a given set of $\mathcal{K}$ nodes is zero if the \expmethod is completely faithful.
Without loss of generality, we use a binary sensitive attribute $s$ (\eg $\textrm{gender}\in\textrm{\{male, female\}}$).

\xhdr{Theorem 5} \textit{Given a node $u$, a sensitive attribute $s$, and a set $\mathcal{K}$ comprising of node $u$ and its perturbations, the group fairness property (Sec.~\ref{sec:def_fair}, Eqn.~\ref{eq:group_fair}) of an explanation $E_{u}$ corresponding to node $u$ can be bounded as follows:}
\begin{equation}
    |~\text{SP}(\mathbf{\hat{y}}_{\mathcal{K}}) - \text{SP}(\mathbf{\hat{y}}_{\mathcal{K}}^{E_u})~| \leq \sum_{\mathclap{s \in \{0, 1\}}}|\text{Err}_{D_{s}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))|,
    \label{eq:lg_unfairness}
\end{equation}
where $\text{SP}(\mathbf{\hat{y}}_{\mathcal{K}})$ and $\text{SP}(\mathbf{\hat{y}}^{E_{u}}_{\mathcal{K}})$ are statistical parity estimates as defined in Sec.~\ref{sec:def_fair}, $D$ is the joint distribution over the node attributes $\mathbf{x}_{u'}$ in graph $\mathcal{G}_{u'}$ and their respective labels $\mathbf{y}_{u'}$ for all nodes $u' \in \mathcal{K}$, $D_{s}$ is the conditional distribution of $D$ given a particular value of the sensitive attribute $s$, and $\text{Err}_{D}(\cdot)=\mathbb{E}_{D}[\mathbf{y}_{u'}-f(\mathcal{G}_{u'})]$ is the error of the model $f$ under the joint distribution $D$.

\textit{Proof Sketch.~} We show that group fairness of an \expmethod is bounded by the sum of the errors $\text{Err}_{D}(\cdot)$ of model $f$ under distribution $D$ conditioned on it's different sensitive attribute values. For a set of $\mathcal{K}$ nodes, the error is computed by taking the expectation of the difference between their true labels, set of model predictions using the original node attributes (\ie node features and incident edges), and their corresponding predictions using the explanation $E_{u}$. Details are in Appendix~\ref{app:lg_unfairness_theory}.

\subsubsection{Counterfactual Fairness}
\label{sec:counter-unfairness-theory}
Analogous to the stability analysis (Sec.~\ref{sec:instability-theory}), we now derive the bounds for counterfactual fairness of the corresponding algorithms.

\xhdr{Theorem 6 (Gradients)} \textit{Given a non-linear activation function $\sigma$ that is Lipschitz continuous, the counterfactual fairness property (Sec.~\ref{sec:def_fair}, Eqn.~\ref{eq:count_fair}) of an explanation $E_{u}$ returned by Gradients method can be bounded as follows:}
% explanation $E_{u}$ returned by the Gradients method is counterfactually fair, \ie}
% the gradient explanation for an original node and its corresponding counterfactual is counterfactually fair, \ie}
% \vspace*{-\abovedisplayskip}
\begin{equation}
    ||\triangledown_{\mathbf{x}_{u^{s}}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq \gamma_{3},
    \label{eq:counter_grad}
\end{equation}
where $\mathbf{x}_{u}$ is node $u$ features and $\mathbf{x}_{u^{s}}$ is the generated counterfactual by flipping $\mathbf{x}_{u}$'s sensitive feature.

\textit{Proof Sketch.~} The $p$-norm distance between $\mathbf{x}_{u^{s}}$ and $\mathbf{x}_{u}$ is one as all the individual node attributes are the same except the sensitive attribute which is flipped (either from $0\to1$ or $1\to0$). The left term in Eqn.~\ref{eq:counter_grad} is similar to Eqn.~\ref{eq:grad_stable} of Theorem 2.
Hence, using $||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p}{=}1$ in Eqn.~\ref{eq:grad_stable}, we obtain the equation in Theorem 6.
% Given a concatenated representation of nodeuandv, explanationEu270returned by the GraphMASK method for layerlis stable, i.e.,

\xhdr{Theorem 7 (GraphMASK)} \textit{Given concatenated embeddings node $u$ and $v$, the counterfactual fairness property (Sec.~\ref{sec:def_fair}, Eqn.~\ref{eq:count_fair}) of an explanation $E_{u}$ returned by GraphMASK method can be bounded as follows:}
% explanation $E_{u}$ returned by the GraphMASK method for layer $l$ is counterfactually fair, \ie} 
% the original and perturbed graph, the scalar location explanation for an edge in layer $l$ is counterfactually fair, \ie}
% \vspace*{-\abovedisplayskip}
\begin{equation}
    ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq \gamma_{4}^{l}~||\mathbf{q}^{l}_{u^{s},v} - \mathbf{q}^{l}_{u,v}||_{2},
    \label{eq:gmask_counter}
\end{equation}
where $\gamma_{4}^{l}$ is the same constant as defined in Theorem 3.

\textit{Proof Sketch.~} A counterfactual node $u^{s}$ is generated by flipping/modifying one sensitive attribute from $\mathbf{x}_{u}$. The left term in Eqn.~\ref{eq:gmask_counter} is similar to Eqn.~\ref{eq:gmask_stable} of Theorem 3. The term $\mathbf{q}^{l}_{u^{s}}$ denotes the counterfactual embedding for node $u^{s}$. Note, for the first layer, the right term of Eqn.~\ref{eq:gmask_counter} simplifies to just $\gamma_{4}^{l}$ as the $p$-norm between the $\mathbf{x}_{u^{s}}$ and $\mathbf{x}_{u}$ is one, \ie $||\mathbf{x}_{u^{s}}{-}\mathbf{x}_{u}||_{p}{=}1$.

\xhdr{Theorem 8 (GraphLIME)} \textit{Given the centered Gram matrices for the original and counterfactual node attributes, the counterfactual fairness property (Sec.~\ref{sec:def_fair}, Eqn.~\ref{eq:count_fair}) of an explanation $E_{u}$ returned by GraphLIME method can be bounded as follows:}
% explanation $E_{u}$ returned by the GraphLIME method for the $k$-th node feature is counterfactually fair, \ie}
% \vspace*{-\abovedisplayskip}
\begin{equation}
    ||\beta^{s}_{k} - \beta_{k}||_{F} \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{\bar{W}}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
    % ||\text{GLIME}(\mathbf{K}^{(k)^{s}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{\bar{W}}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
\end{equation}
where $E_{u}$ is a node mask produced using the attribute importance $\beta^{'}_{k}$ and $\beta^{s}_{k}$ is the attribute importance generated by GraphLIME for the $k$-th attribute of node $u^{s}$.

\textit{Proof Sketch.~} Let us consider the $k$-th node attribute a binary sensitive attribute where $s \in \{0, 1\}$. Similar to stability, in counterfactual fairness we obtain a matrix $\mathbf{W}$ where $\eta$ will be either $1$ or $-1$, \ie $\eta{=}1$ when flipping the sensitive attribute from $0 \to 1$, and $\eta{=}{-}1$ when flipping from $1 \to 0$. This does not change the positive semidefinite and invertible property of $\mathbf{W}$ as all diagonal elements are still 1 (\ie invertible) and the off-diagonal elements are exponential which are always positive. We denote this modified matrix as $\mathbf{\bar{W}}$.
The proof has a similar structure as Theorem 4.
% \marinka{Is the full proof in Appendix--where? Let's use original/reference names for GNN explanation methods. GraphLIME paper does not use GLIME.}
% \chirag{the counterfactual proofs are in the main tex as they are specific cases of stability. I agree with the GLIME thing. the equations were getting a bit longer so i abbreviated them. I will fix this once I kick-off the PGMExplainer experiments in background.}
% \chirag{Fixed!} \chirag{will discuss about the new form and then update the appendix accordingly}
%%%%%%%%%
%% EVERYTHING BELOW IS COMMENTED SECTION OF THE ORIGINAL PROOF FOR FAIRNESS and STABILITY FOR REFERENCE.
% \subsection{Local-Group Unfairness of known GNN Explainers}
% \label{sec:local_group_fair}
% % \marinka{Can we move this section up and make it Section 5.2? So that we start with the analysis that applies broadly to all known explainers and the proceed with the analysis of representative methods?}\chirag{Sounds better. Done}
% A model satisfies group fairness if the instances in the protected and unprotected groups have equal probability of being assigned to the positive predicted class. In this context, the unfairness property is dependent on the faithfulness of an explanation algorithm, \ie the local-group unfairness of node $u$ for a given set of $\mathcal{K}$ nodes is zero if the explanation algorithm is completely faithful.
% % as the explanations generate the same predictions as the original model. 
% Without loss of generality, we consider a binary sensitive attribute $s$ (\eg gender $\in$ \{male, female\}).
% \xhdr{Theorem 2 (Local-Group Unfairness)} \textit{Given node $u$, its sensitive attribute $s$, and a set of $\mathcal{K}$ perturbations, the explanation for node $u$ satisfies local-group fairness if:}
% \begin{equation}
%     |\text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'})| \leq \sum_{s \in \{0, 1\}}|\text{Err}_{D_{s}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))|
%     % \text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'}) \leq \sum_{s \in \{0, 1\}}\text{Err}_{D_{s}}\big(f(t(E_{u}, \mathcal{G}_{u'})) - f(\mathcal{G}_{u'})\big),
% \end{equation}
% where $D$ is the joint distribution over the node attributes $\mathbf{x}_{u'}$ in graph $\mathcal{G}_{u'}$ and their respective labels $\mathbf{y}_{u'}$ for all nodes $u' \in \mathcal{K}$, $D_{s}$ is the conditional distribution of $D$ given a particular value of the sensitive attribute $s$, and $\text{Err}_{D}(\cdot)=\mathbb{E}_{D}[\mathbf{y}_{u'}-f(\mathcal{G}_{u'})]$ is the error of the model $f$ under the joint distribution $D$.

% \textit{Proof Sketch.~} We show that the local-group unfairness of any explanation method is bounded by the sum of the error $\text{Err}_{D}(\cdot)$ of model $f$ under distribution $D$ conditioned on different values of its sensitive attribute. For the set of $\mathcal{K}$ nodes, the error is computed by taking the expectation of the difference between their respective true labels, set of model predictions using the original input attributes (\ie node features and incident edges), and their corresponding predictions using the explanation masks. See Sec.~\ref{app:local_group_fair} for more details.


% % \textit{Proof.~} For local-group unfairness, we define the total variation divergence $d_{\text{TV}}$ to measure the difference between two probability distributions, \ie $\mathbf{y}_{u'}$ and $\mathbf{\hat{y}}_{u'}$. For a given binary sensitive attribute $s \in \{0, 1\}$, we can write:~ $d_{\text{TV}}(D_{s}(\mathbf{y}_{u'}), D_{s}(\mathbf{\hat{y}}_{u'})) \leq \mathbb{E}_{D_{s}}[|\mathbf{y}_{u'}-f(\mathcal{G}_{u'})|]$ \cite{zhao2019inherent}.
% % The total variation divergence is symmetrical and satisfies triangle inequality. Hence, we have:
% % \begin{align*}
% %     \begin{split}
% %         d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{1}(\mathbf{y}_{u'})) \leq d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{0}(\mathbf{\hat{y}}_{u'})){+}d_{\text{TV}}(D_{0}(\mathbf{\hat{y}}_{u'}), D_{1}(\mathbf{\hat{y}}_{u'})){+}\\d_{\text{TV}}(D_{1}(\mathbf{y}_{u'}), D_{1}(\mathbf{\hat{y}}_{u'}))
% %     \end{split}
% % \end{align*}

% % Now, the middle term in the right side of the inequality is the statistical parity (SP) for the binary sensitive attribute and therefore we can simplify the equation as:
% % \begin{equation}
% %     d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{1}(\mathbf{y}_{u'})) \leq d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{0}(\mathbf{\hat{y}}_{u'})){+}\text{SP}(\mathbf{\hat{y}}_{u'}){+}\\d_{\text{TV}}(D_{1}(\mathbf{y}_{u'}), D_{1}(\mathbf{\hat{y}}_{u'}))
% %     \label{eq:dtv_original}
% % \end{equation}

% % Similarly, using the explanation $E$, we can write a similar inequality of the local-group predictions $\mathbf{\hat{y}}^{E}_{u'}$ and equate the left hand side terms to get:
% % \begin{equation}
% %     \begin{split}
% %         d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{0}(\mathbf{\hat{y}}_{u'})){+}\text{SP}(\mathbf{\hat{y}}_{u'}){+}d_{\text{TV}}(D_{1}(\mathbf{y}_{u'}), D_{1}(\mathbf{\hat{y}}_{u'})) = d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{0}(\mathbf{\hat{y}}^{E}_{u'}))\\{+}\text{SP}(\mathbf{\hat{y}}^{E}_{u'}){+}d_{\text{TV}}(D_{1}(\mathbf{y}_{u'}), D_{1}(\mathbf{\hat{y}}^{E}_{u'}))
% %     \end{split}
% %     \label{eq:lg_fairness_equate}
% % \end{equation}

% % Using Lemma 3.1 of \cite{zhao2019inherent}, we can write $d_{\text{TV}}(D_{s}(\mathbf{y}_{u'}), D_{s}(\mathbf{\hat{y}}_{u'})) \leq \text{Err}_{D_{s}}(f(\mathcal{G}_{u'}))$. Further simplification of Eqn.~\ref{eq:lg_fairness_equate} and plugging the lemma, we get:
% % \begin{eqnarray}
% %     \begin{split}
% %         \text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'}){=} d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{0}(\mathbf{\hat{y}}^{E}_{u'})){-}d_{\text{TV}}(D_{0}(\mathbf{y}_{u'}), D_{0}(\mathbf{\hat{y}}_{u'}))\\{+}d_{\text{TV}}(D_{1}(\mathbf{y}_{u'}), D_{1}(\mathbf{\hat{y}}^{E}_{u'})){-}d_{\text{TV}}(D_{1}(\mathbf{y}_{u'}), D_{1}(\mathbf{\hat{y}}_{u'}))
% %     \end{split}\\
% %     \begin{split}
% %         \text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'})\leq \text{Err}_{D_{0}}(f(t(E_{u},\mathcal{G}_{u'}))){-}\text{Err}_{D_{0}}(f(\mathcal{G}_{u'})){+}\text{Err}_{D_{1}}(f(t(E_{u},\mathcal{G}_{u'}))){-}\\\text{Err}_{D_{1}}(f(\mathcal{G}_{u'}))
% %     \end{split}\\
% %     \text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'})\leq \text{Err}_{D_{0}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'})){+}\text{Err}_{D_{1}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))
% % \end{eqnarray}

% % Taking the absolute value as norms on both sides, we get:
% % \begin{align*}
% %     & |\text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'})|\leq |\text{Err}_{D_{0}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'})){+}\text{Err}_{D_{1}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))|\\
% %     & |\text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'})| \leq |\text{Err}_{D_{0}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))|+|\text{Err}_{D_{1}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))| \tag{Using triangle inequality} \\
% %     & |\text{SP}(\mathbf{\hat{y}}^{E}_{u'}){-}\text{SP}(\mathbf{\hat{y}}_{u'})| \leq \sum_{s \in \{0, 1\}}|\text{Err}_{D_{s}}(f(t(E_{u},\mathcal{G}_{u'})){-}f(\mathcal{G}_{u'}))|
% % \end{align*}


% % For the set of $\mathcal{K}$ nodes, we define two subsets $m^{+}$ and $m^{-}$ that contains nodes from set $\mathcal{K}$ that were correctly and incorrectly classified by the explanation method respectively. Considering the \textit{gender} attribute as an example, let us define $p$ and $q$ as the probability of an instance being `female' in sets $m^{+}$ and $m^{-}$. Thus, the probability of the sensitive attribute being a `male' in these sets are $(1-p)$ and $(1-q)$, respectively.

% \subsection{Explainers using Surrogate Models: GraphLIME}\label{sec:graphlime}

% GraphLIME \cite{huang2020graphlime} is a local interpretable model explanation for GNNs that identifies a nonlinear interpretable model over the neighbors of a node that is locally faithful to the node's prediction.
% It considers a feature-wise kernelized nonlinear method called Hilbert-Schmidt Independence Criterion Lasso (HSIC Lasso) as an explanation model.

% \xhdr{Setup} For each node prediction, the HSIC Lasso objective function is defined as:
% \begin{equation}
%     \min_{\beta \in \mathbb{R}^{d}} \frac{1}{2} || \mathbf{L} - \sum_{k=1}^{M} \beta_{k} \mathbf{K}^{(k)} ||^{2}_{F} + \rho||\beta||_{1},
%     \label{eq:hsic}
% \end{equation}
% where $||\cdot||_{F}$ is the Frobenius norm, $\rho \geq 0$ is the regularization parameter, $||\cdot||_{1}$ is the $l_{1}$ norm to enforce sparsity, $\mathbf{L}$ is the centered Gram matrix, $L_{ij} = L(y_{i}, y_{j})$ is the kernel for the output labels of the nodes, $\mathbf{K}^{k}$ is the centered gram matrix for the $k$-th feature, and $K_{ij}=K(x_{i}^{(k)}, x_{j}^{(k)})$ is the kernel for the $k$-th dimensional input node features $\mathbf{x}_{u}$.
% We use Gaussian kernel for both input and the predictions of all neighbors of node $u$.
% \begin{equation}
%     \begin{split}
%         K(x_{i}^{(k)}, x_{j}^{(k)}) = \exp \big( - \frac{(x_{i}^{(k)}-x_{j}^{(k)})^{2}}{2\sigma_{x}^{2}} \big); 
%         L(y_{i}^{(k)}, y_{j}^{(k)}) = \exp \big( - \frac{||y_{i}^{(k)}-y_{j}^{(k)}||^{2}_{2}}{2\sigma_{y}^{2}} \big),
%     \end{split}
% \end{equation}
% The HSIC Lasso objective can be regarded as a minimum redundancy maximum relevancy (mRMR) based feature selection method \cite{peng2005minimum}. Eqn.~\ref{eq:hsic} can be rewritten as:
% \begin{equation}
%     || \mathbf{L} - \sum_{\mathclap{k=1}}^{\mathclap{M}} \beta_{k} \mathbf{K}^{(k)} ||^{2}_{F} = \text{HSIC}(\mathbf{y}, \mathbf{y}) + \sum_{\mathclap{i=1}}^{\mathclap{M}}\beta_{i}\text{HSIC}(\mathbf{x}_{i}, \mathbf{y}) + \sum_{\mathclap{i,j=1}}^{\mathclap{M}}\beta_{i}\beta_{j}\text{HSIC}(\mathbf{x}_{i}, \mathbf{x}_{j}),
% \end{equation}
% where HSIC$(\mathbf{x}_{i}, \mathbf{y}) = \text{tr}(\mathbf{K}^{(k)}, \mathbf{L})$ is a kernel-based independence measure called the (empirical) Hilbert-Schmidt independence criterion (HSIC) \cite{gretton2005measuring}.
% % The empirical HSIC converges to the true HSIC with $O(1/\sqrt{N})$ (see Theorem 3 in \cite{gretton2005measuring}). 
% Further, the HSIC lasso is a convex optimization problem \cite{yamada2014high} and hence given a set of features it will learn feature importance that fit to the predicted labels. We now derive the upper bound for the explanation generated by GraphLIME (or simply GLIME) for the $k$-th node feature. We exclude the sparsity regularizer in our analysis as GLIME enforces sparsity by selecting the top-$P$ features after the optimization.

% % where HSIC(uk, y) = tr(K¯ (k)L¯) is a kernel-based independence measure called the (empirical) Hilbert-Schmidt independence criterion (HSIC) (Gretton et al., 2005) and tr(·) denotes the trace. HSIC(y, y) is a constant and can be ignored. HSIC always takes a non-negative value, and is zero if and only if two random variables are statistically independent when a universal reproducing kernel (Steinwart, 2001) such as the Gaussian kernel is used. Note that the empirical HSIC asymptotically converges to the true HSIC with O(1/√n) (see Theorem 3 in Gretton et al. (2005)). In addition, HSIC can be regarded as the centered version of the kernel target alignment (KTA) (Shawe-Taylor and Kandola, 2002)

% \xhdr{Theorem 3 (GraphLIME Instability)} \textit{Given the centered Gram matrix for the original and perturbed set of node features, the explanation for the $k$-th feature of GLIME is stable if:}
% \begin{equation}
%     ||\text{GLIME}(\mathbf{K}^{(k)^{'}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
% \end{equation}
% where $\gamma_{2}=\text{tr}(\mathbf{\bar{L}})~\text{tr}((\mathbf{K}^{(k)})^{-1})$ is a constant independent of the added noise and $\mathbf{W}$ is a matrix comprising of the added noise terms.

% \textit{Proof Sketch.~} We prove that the instability of GLIME is bounded by the trace of the Gram matrix for the output label and of the perturbed Gram matrix due to the noise added in the input graph. We first derive the closed-form of the feature importance coefficient $\beta$ and then use it derive the upper bounds for the instability of GLIME. See Sec.~\ref{app:graphlime} for more details.

% % Note, $||Q||_{F}^{2} = \text{tr}(QQ^{T}) = \text{tr}(QQ)$, where $Q$ is a symmetric matrix and tr($\cdot$) is the trace of the matrix.
% % The objective function can be simplified as:
% % \begin{align*}
% %     & \frac{1}{2} || \mathbf{L} - \sum_{i=1}^{M} \beta_{i} \mathbf{K}^{(i)} ||^{2}_{F} \\
% %     & = \frac{1}{2} \text{tr}\big( (\mathbf{L}-\sum_{i=1}^{M} \beta_{i} \mathbf{K}^{(i)}) \cdot (\mathbf{L}^{T}-\sum_{i=1}^{M} \beta_{i} \mathbf{K}^{(i)^{T}}) \big) \\
% %     & = \frac{1}{2} \text{tr}\big( (\mathbf{L}-\sum_{i=1}^{M} \beta_{i} \mathbf{K}^{(i)}) \cdot (\mathbf{L}^{T}-\sum_{i=1}^{M} \beta_{i} \mathbf{K}^{(i)}) \big) \\
% %     & = \frac{1}{2} \text{tr}\big( \mathbf{L}\mathbf{L}^{T}-2\sum_{i=1}^{M} \beta_{i} \mathbf{L}\mathbf{K}^{(i)} + \sum_{i,j=1}^{M} \beta_{i}\beta_{j}\mathbf{K}^{(i)}\mathbf{K}^{(j)} \big)
% % \end{align*}
% % We want to minimize the above objective function $O$. We take the partial derivative of $O$ $w.r.t.$ $\beta_{k}$:
% % % Both $\mathbf{L}$ and $\mathbf{K}^{(k)}$ are symmetric matrices and hence,
% % % \begin{equation}
% % %     \frac{\partial{O}}{\partial{\beta_{k}}} = -\mathbf{L}\mathbf{K}^{(k)} + \sum_{j=1}^{d}\beta_{j}\mathbf{K}^{(j)}\mathbf{K}^{(k)} = 0
% % % \end{equation}
% % \begin{align*}
% %     & \frac{\partial{O}}{\partial{\beta_{k}}} = -\mathbf{L}\mathbf{K}^{(k)} + \sum_{j=1}^{M}\beta_{j}\mathbf{K}^{(j)}\mathbf{K}^{(k)} = 0\\
% %     & \implies -\mathbf{L}\mathbf{K}^{(k)} + \sum_{j=1}^{M}\beta_{j}\mathbf{K}^{(j)}\mathbf{K}^{(k)} = 0\\
% %     & \implies (-\mathbf{L} + \sum_{j=1}^{M}\beta_{j}\mathbf{K}^{(j)})\mathbf{K}^{(k)} = 0 \\
% %     & \implies (-\mathbf{L} + \sum_{j=1;j\neq k}^{M}\beta_{j}\mathbf{K}^{(j)} + \beta_{k}\mathbf{K}^{(k)})\mathbf{K}^{(k)} = 0 \\
% % \end{align*}
% % We finally get,
% % \begin{equation}
% %     \beta_{k}\mathbf{K}^{(k)} = \mathbf{L} - \sum_{j=1;j\neq k}^{M}\beta_{j}\mathbf{K}^{(j)}
% % \end{equation}
% % The gram matrix is invertible as it is a full rank symmetric matrix with all the diagonal elements as $1$ (since $K(x_{i},x_{i}) = 1$) and so:
% % \begin{equation}
% %     \beta_{k}=\mathbf{\bar{L}}(\mathbf{K}^{(k)})^{-1},
% % \end{equation}
% % where $\mathbf{\bar{L}}=\mathbf{L}-\sum_{j=1;j\neq k}^{M}\beta_{j}\mathbf{K}^{(j)}$.

% % On adding infinitesimal noise $\eta$ to the $k$-th feature, we obtain a new gram matrix given by: $\mathbf{K}^{(k)^{'}} = \mathbf{K}^{(k)}\circ \mathbf{W}$, where $\mathbf{W}\in \mathbb{R}^{M\times M}$ is a function of $\eta$ and $x_{i}$. 
% % For instance, adding noise $\eta$ to $x_{i}^{(k)}$, we get $K^{'}(x_{i}^{(k)}, x_{j}^{(k)})$ as:
% % \begin{align*}
% %     & K^{'}(x_{i}^{(k)}, x_{j}^{(k)}) = \exp \big( - \frac{(x_{i}^{(k)}+\eta-x_{j}^{(k)})^{2}}{2\sigma_{x}^{2}} \big)\\
% %     & = \exp \big( - \frac{(x_{i}^{(k)}-x_{j}^{(k)})^{2} + \eta^{2} + 2\eta(x_{i}^{(k)}-x_{j}^{(k)})}{2\sigma_{x}^{2}} \big)\\
% %     & = \exp \big( -\frac{(x_{i}^{(k)}-x_{j}^{(k)})^{2} + 2\eta(x_{i}^{(k)}-x_{j}^{(k)})}{2\sigma_{x}^{2}} \big) \tag{$\eta^{2}=0$ as $\eta$ is infinitesimal noise} \\
% %     & = \exp \big( -\frac{(x_{i}^{(k)}-x_{j}^{(k)})^{2}}{2\sigma_{x}^{2}} \big)\cdot \exp \big( -\frac{2\eta(x_{i}^{(k)}-x_{j}^{(k)})}{2\sigma_{x}^{2}} \big)
% % \end{align*}

% % The importance for the $k$-th node feature is generated by GraphLIME (GLIME) as $\beta_{k}$.
% % We can now represent the Frobenius norm of the difference between the explanations from GLIME for the original and noisy graph as:
% % % \begin{eqnarray}
% % %     ||\text{GLIME}(\mathbf{K}^{(k)^{'}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} = ||\mathbf{L}(\mathbf{K}^{(k)^{'}})^{-1} - \mathbf{L}(\mathbf{K}^{(k)})^{-1}||_{F}
% % % \end{eqnarray}
% % \begin{align*}
% %     & ||\text{GLIME}(\mathbf{K}^{(k)^{'}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} = ||\mathbf{\bar{L}}(\mathbf{K}^{(k)^{'}})^{-1} - \mathbf{\bar{L}}(\mathbf{K}^{(k)})^{-1}||_{F}\\
% %     & = ||\mathbf{\bar{L}}\big((\mathbf{K}^{(k)^{'}})^{-1} - (\mathbf{K}^{(k)})^{-1}\big)||_{F}\\
% %     & \leq ||\mathbf{\bar{L}}||_{F}~||(\mathbf{K}^{(k)^{'}})^{-1}-(\mathbf{K}^{(k)})^{-1}||_{F} \tag{Using Cauchy-Schwartz inequality}\\
% %     & \leq ||\mathbf{\bar{L}}||_{F}~||(\mathbf{K}^{(k)}\circ \mathbf{W})^{-1}-(\mathbf{K}^{(k)})^{-1}||_{F}\\
% %     & \leq ||\mathbf{\bar{L}}||_{F}~||(\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}}\mathbf{K}^{(k)})^{-1}-(\mathbf{K}^{(k)})^{-1}||_{F}, \tag{Using Theorem 3.1 from \cite{reams1999hadamard}}\\
% % \end{align*}
% % where $\mathbf{e}$ is a $m \times 1$ vector of all ones. Note, for using Theorem 3.1 from \cite{reams1999hadamard} we need: 1) $\mathbf{K}^{(k)}$ is positive semidefinite; and 2) $\mathbf{W}$ is positive definite or is
% % almost positive definite and invertible.
% % (1) is true by definition as $\mathbf{K}^{(k)}$ is a gram matrix and they are positive semidefinite.
% % For (2), let us consider a case where $\mathbf{W} \in \mathbb{R}^{2 \times 2}$. Using the Gaussian kernel $\mathbf{K}^{(k)}$, the perturbed gram matrix $\mathbf{K}^{(k)^{'}}$ is:
% % \begin{align*}
% %     & \mathbf{K}^{(k)^{'}} = \begin{bmatrix} 1 & \exp \big({-}\frac{(x_{1}^{(k)}{-}x_{2}^{(k)})^{2}}{2\sigma_{x}^{2}} \big) \cdot \exp \big( {-}\frac{2\eta(x_{1}^{(k)}{-}x_{2}^{(k)})}{2\sigma_{x}^{2}} \big)\\
% %     \exp \big({-}\frac{(x_{1}^{(k)}-x_{2}^{(k)})^{2}}{2\sigma_{x}^{2}} \big) \cdot \exp \big( {-}\frac{2\eta(x_{1}^{(k)}{-}x_{2}^{(k)})}{2\sigma_{x}^{2}} \big) & 1\end{bmatrix}\\
% %     & = \begin{bmatrix} 1 & \exp \big( {-}\frac{(x_{1}^{(k)}{-}x_{2}^{(k)})^{2}}{2\sigma_{x}^{2}} \big)\\
% %     \exp \big({-}\frac{(x_{1}^{(k)}{-}x_{2}^{(k)})^{2}}{2\sigma_{x}^{2}} \big) & 1\end{bmatrix} \circ \begin{bmatrix} 1 & \exp \big( {-}\frac{2\eta(x_{1}^{(k)}{-}x_{2}^{(k)})}{2\sigma_{x}^{2}} \big)\\
% %     \exp \big({-}\frac{2\eta(x_{1}^{(k)}{-}x_{2}^{(k)})}{2\sigma_{x}^{2}} \big) & 1\end{bmatrix}
% % \end{align*}
% % Hence, $\mathbf{W}$ is:
% % \begin{equation}
% %     \mathbf{W} = \begin{bmatrix} 1 & \exp \big( {-}\frac{2\eta(x_{1}^{(k)}{-}x_{2}^{(k)})}{2\sigma_{x}^{2}} \big)\\
% %     \exp \big( {-}\frac{2\eta(x_{1}^{(k)}{-}x_{2}^{(k)})}{2\sigma_{x}^{2}} \big) & 1\end{bmatrix}
% % \end{equation}
% % For positive definite, we need to show $b^{T}\mathbf{W}b > 0$ for any non-zero vector $b$. 
% % All the elements of $\mathbf{W}$ are positive and using a $b$ vector with all ones will result in $b^{T}\mathbf{W}b > 0$. Hence, $\mathbf{W}$ is positive definite. 
% % Now, both $\mathbf{W}$ and $\mathbf{K}^{(k)}$ are invertible matrix so we can use the property $(AB)^{-1}=B^{-1}A^{-1}$. Putting everything together we get:
% % \begin{align*}
% %         & ||\text{GLIME}(\mathbf{K}^{(k)^{'}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} \leq ||\mathbf{\bar{L}}||_{F}~||(\mathbf{K}^{(k)})^{-1}(\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-(\mathbf{K}^{(k)})^{-1}||_{F}\\
% %         & \leq ||\mathbf{\bar{L}}||_{F}~||(\mathbf{K}^{(k)})^{-1}\big((\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I}\big)||_{F}\\
% %         & \leq ||\mathbf{\bar{L}}||_{F}~||(\mathbf{K}^{(k)})^{-1}||_{F}~||(\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I}||_{F} \tag{Using Cauchy-Schwartz inequality}\\
% %         & \leq \text{tr}(\mathbf{\bar{L}})~\text{tr}((\mathbf{K}^{(k)})^{-1})~\text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I})\\
% %         & \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{W}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
% %         % & \leq \sqrt{\text{rk}(\mathbf{\bar{L}})}~||\mathbf{\bar{L}}||_{2}~\sqrt{\text{rk}((\mathbf{K}^{(k)})^{-1})}~||(\mathbf{K}^{(k)})^{-1}||_{2}
% % \end{align*}
% % where $\gamma_{2}=\text{tr}(\mathbf{\bar{L}})~\text{tr}((\mathbf{K}^{(k)})^{-1})$ is a constant independent of the added noise.

% \xhdr{Theorem 4 (GraphLIME Counterfactual Unfairness)} \textit{Given the centered Gram matrix for the original and counterfactual set of node features, the GLIME explanation is counterfactually fair if:}
% \begin{equation}
%     ||\text{GLIME}(\mathbf{K}^{(k)^{s}}) - \text{GLIME}(\mathbf{K}^{(k)})||_{F} \leq \gamma_{2}~\cdot~ \text{tr}((\frac{1}{\mathbf{e}^{T}\mathbf{\bar{W}}^{-1}\mathbf{e}})^{-1}-\mathbf{I}),
% \end{equation}
% where $\mathbf{K}^{(k)^{s}}$ is the counterfactual version of the original gram matrix.

% \textit{Proof Sketch.~} Let us consider the $k$-th node feature a binary sensitive attribute where $s \in \{0, 1\}$. Similar to stability, in counterfactual fairness we obtain a matrix $\mathbf{W}$ where $\eta$ will be either $1$ or $-1$, \ie $\eta{=}1$ when flipping the sensitive attribute from $0 \to 1$, and $\eta{=}{-}1$ when flipping from $1 \to 0$. This does not change the positive semidefinite and invertible property of $\mathbf{W}$ as all diagonal elements are still 1 (\ie invertible) and the off-diagonal elements are exponential which are always positive. We denote this modified matrix as $\mathbf{\bar{W}}$.
% The proof has a similar form as Theorem 3 and can be proved analogously.

% \subsection{Explainers using Gradients: GNN Gradients}\label{sec:gradient}

% Gradient \cite{Simonyan14a} based explanation generate local explanations for the prediction of a differentiable model $f$ using its gradient with respect to the node features $\mathbf{x}_{u}$: $\triangledown_{\mathbf{x}_{u}}f$. Intuitively, gradient represents how much difference a tiny change in each feature of a node $u$ would make to its corresponding classification score.
% We now take the vanilla gradient form of gradient explanations and derive the upper bounds for its instability and counterfactual unfairness.

% \xhdr{Theorem 5 (Gradient Instability)} \textit{Given a non-linear activation function $\sigma$ that is Lipschitz continuous, the gradient explanation for an original and perturbed graph is stable if:}
% \begin{equation}
%     ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq \gamma_{3}||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p},
%     \label{eq:grad_stable}
% \end{equation}
% where $\gamma_{3}$ is a constant, $\mathbf{x}_{u}$ is the original node feature, and $\mathbf{x}_{u'}$ is the perturbed node feature.

% \textit{Proof Sketch.~} We prove that gradient explanations are Lipschitz using data processing inequalities and the Lipschitz constant is the product of the $l_{\text{p}}$-norm of the difference in the predictions between the original and perturbed node, the weight of the last classification layer, and the weights associated with node $u$ itself. See Sec.~\ref{app:gradient} for more details.

% % Similar to Sec.~\ref{sec:local_group_faith}, let us consider a two-layer GNN model trained on a node classification task using softmax cross-entropy loss function with the first layer a message-passing GNN layer and the second layer as a fully-connected layer. The cross-entropy (CE) loss is given as:
% % \begin{equation}
% %     \text{CE} = -\sum_{i} y_{i}\log \hat{y}_{u},  % \hat{y}_{i},
% % \end{equation}
% % where $\mathbf{y}$ is a vector with one one non-zero element (which is 1), $\mathbf{\hat{y}}_{u}{=}\text{softmax}(\mathbf{h}_{u}^{2})$, $\mathbf{h}_{u}^{2}{=}\mathbf{W}_{\text{fc}}\mathbf{h}_{u}^{1} + \mathbf{b}$, and $\mathbf{h}_{u}^{1}{=}\text{sp}(\mathbf{W}_{a}^{1}\mathbf{x}_{u} + \mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v})$.
% % $\mathbf{W}_{n}^{1}$ is the weight matrix associated with the neighbors of node $u$ and $\mathbf{W}_{a}^{1}$ is the self-attention weight matrix at layer one.
% % For the fully-connected layer, we have $\mathbf{W}_{\text{fc}}$ as the weight matrix and $\mathbf{b}$ as the bias term.
% % ``sp'' is the softplus activation function which is a smooth approximation of the ReLU function.
% % For stability, we generate $\mathbf{x}_{u'}$ by adding noise to the node features of node $u$ and keep everything else constant. Therefore, $\mathbf{h}_{u'}^{1} = \text{sp}(\mathbf{W}_{a}^{1}\mathbf{x}_{u'}+\mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v})$.
% % Now, the differentiation of the model \textit{w.r.t.} the node features can be given as:
% % \begin{align*}
% %     \triangledown_{\mathbf{x}_{u}}f = \deriv{(\text{CE})}{\mathbf{x}_{u}} = \deriv{(\text{CE})}{\mathbf{h}_{u}^{2}}\deriv{\mathbf{h}_{u}^{2}}{\mathbf{h}_{u}^{1}}\deriv{\mathbf{h}_{u}^{1}}{\mathbf{x}_{u}}, \tag{By chain rule}
% % \end{align*}
% % Note, the advantage of using \textit{softplus} activation function is that it is differentiable for all $x$, \ie
% % \begin{align*}
% %     & \text{sp}(x)=\textit{ln}(1+\exp^{x}) \\
% %     & \deriv{(\text{sp}(x))}{\text{x}} = \frac{\exp^{x}}{1 + \exp^{x}} \cdot \frac{(1/\exp^{x})}{(1/\exp^{x})}\\
% %     & = \frac{1}{1 + \exp^{-x}}\\
% %     & = \sigma(x),
% % \end{align*}
% % where $\sigma(\cdot)$ is the sigmoid activation function. Putting it all together we get,
% % \begin{eqnarray}
% %     \triangledown_{\mathbf{x}_{u}}f = (\mathbf{y}_{u}-\mathbf{\hat{y}}_{u})(\mathbf{W}_{\text{fc}})^{T}\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u} + \mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}_{u}} \mathbf{x}_{v})(\mathbf{W}_{a}^{1})^{T}\\
% %     \triangledown_{\mathbf{x}_{u'}}f = (\mathbf{y}_{u}-\mathbf{\hat{y}}_{u})(\mathbf{W}_{\text{fc}})^{T}\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u'} + \mathbf{W}_{n}^{1}\sum_{v\in \mathcal{N}'_{u}} \mathbf{x}_{v})(\mathbf{W}_{a}^{1})^{T}
% % \end{eqnarray}
% % Note, $\mathbf{\hat{y}}_{u}$ is same for both  original and perturbed node according to the Definition 2 in Sec.~\ref{sec:problem} and we drop the second neighborhood term since the probability ($p_{r}$) of rewiring the edges is very small to maintain the original graph structure.
% % Hence, subtracting the explanations (model gradients) for the original and perturbed node features and taking the norm on both sides, we get:
% % \begin{align*}
% %     & ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} = ||(\mathbf{y}_{u}-\mathbf{\hat{y}}_{u})(\mathbf{W}_{\text{fc}})^{T}\big(\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u'})-\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u})\big)(\mathbf{W}_{a}^{1})^{T}||_{p},\\
% % \end{align*}
% % Using Cauchy-Schwartz inequality, we get:
% % \begin{align*}
% %     & ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u'})-\sigma(\mathbf{W}_{a}^{1}\mathbf{x}_{u})||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}
% % \end{align*}
% % Assuming that $\sigma(\cdot)$ is normalized Lipschitz, \ie $||\sigma{(b)}-\sigma{(a)}||_{p} \leq ||b-a||_{p}$, we get,
% % \begin{align*}
% %     & ||\triangledown_{\mathbf{x}_{u'}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}\mathbf{x}_{u'}-\mathbf{W}_{a}^{1}\mathbf{x}_{u}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}\\
% %     & \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}(\mathbf{x}_{u'}-\mathbf{x}_{u})||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}\\
% %     & \leq ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}||_{p}~||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p} \tag{Using Cauchy-Schwartz inequality}\\
% %     & \leq \gamma_{3}~||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p},
% % \end{align*}
% % where $\gamma_{3} = ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~||\mathbf{W}_{a}^{1}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p}$.
% % For a GNN model with $L$ message-passing layers and one fully-connected layer for node classification, $\gamma_{3}$ takes the general form of:
% % \begin{equation}
% %     \gamma_{3} = ||\mathbf{y}_{u}-\mathbf{\hat{y}}_{u}||_{p}~||(\mathbf{W}_{\text{fc}})^{T}||_{p}~\prod_{l=1}^{L}||\mathbf{W}_{a}^{l}||_{p}~||(\mathbf{W}_{a}^{1})^{T}||_{p},
% %     % \mathcal{C}_{\text{fc}}~||\mathbf{W}_{\text{fc}}||_{2}~\prod_{l=1}^{L}\mathcal{C}_{l}||\mathbf{W}_{a}^{l}||_{2},
% % \end{equation}
% % where $\mathbf{W}_{a}^{l}$ is the self-attention weight associated with the $l$-th message-passing layer.

% \xhdr{Theorem 6 (Gradient Counterfactual Unfairness)} \textit{Given a non-linear activation function $\sigma$ that is Lipschitz continuous, the gradient explanation for an original node and its corresponding counterfactual is counterfactually fair if:}
% \begin{equation}
%     ||\triangledown_{\mathbf{x}_{u^{s}}}f-\triangledown_{\mathbf{x}_{u}}f||_{p} \leq \gamma_{3},
%     \label{eq:counter_grad}
% \end{equation}
% where $\mathbf{x}_{u}$ is the original node feature and $\mathbf{x}_{u^{s}}$ is the generated counterfactual by flipping the sensitive attribute of the original node feature.

% \textit{Proof Sketch.~} The $p$-norm distance between the features of a node and its counterfactual version is one, \ie $||\mathbf{x}_{u^{s}}-\mathbf{x}_{u}||_{p}{=}1$, as all their individual node features are the same except the sensitive attribute which is flipped (either from $0\to1$ or $1\to0$). The left term in Eqn.~\ref{eq:counter_grad} is similar to that of Eqn.~\ref{eq:grad_stable} in Theorem 4.
% Hence, using $||\mathbf{x}_{u'}-\mathbf{x}_{u}||_{p}{=}1$ in Eqn.~\ref{eq:grad_stable}, we obtain the equation in Theorem 5.

% \subsection{Explainers using Perturbations: GraphMASK}\label{sec:graphmask}

% GraphMASK \cite{schlichtkrull2020interpreting} detect edges at each layer $l$ that can be ignored without affecting the output model predictions.
% In general, dropping edges from a given graph is non-trivial, and, hence, for each edge at layer $l$, GraphMASK learns a binary choice $z^{l}_{u, v}$ that indicates whether the edge can be dropped, and then replaces the given edge with a learned baseline. Here, $z^{l}_{u, v}$ indicates an edge connecting node $u$ and $v$.
% GraphMASK learns $z^{l}_{u,v}$ for all $(u,v) \in \mathcal{E}$ for the training data points using an erasure function $g_{\pi}$, where $\pi$ denotes the parameters of $g$.
% For explaining a given prediction, GraphMASK uses this trained function $g_{\pi}$ and generates a masked representation of the graph using: $\Tilde{h}_{u}^{l}{=} \mathbf{Z}^{l}\circ h_{u}^{l} + \alpha^{l}\circ(1-\mathbf{Z}^{l})$,
% % \begin{equation}
% %     \Tilde{h}_{u}^{l}{=} \mathbf{Z}^{l}\circ h_{u}^{l} + \alpha^{l}\circ(1-\mathbf{Z}^{l}),
% % \end{equation}
% where $\mathbf{Z}^{l}$ comprises of all the individual binary scores $z^{l}_{u, v}=g_{\pi}(h_{u}^{l}, h_{v}^{l})$, $\alpha^{l}$ is the learned baseline, and `$\circ$' denotes the element-wise Hadamard product.
% %  which can also be replaced with samples from a Gaussian distribution

% \xhdr{Setup} GraphMASK computes the parameters $\pi$ for the erasure function using fully-connected layers with non-linearity and layer-wise normalization.
% The scalar location parameter $z^{l}_{u, v}$ is given as:
% \begin{equation}
%     z^{l}_{u, v} = \mathbf{W}_{2}^{l}~\text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u,v})),
%     \label{eq:gpi}
% \end{equation}
% where sp is the softplus activation function, LN is the layer normalization function, and $q^{l}_{u,v}$ represents the concatenated representations of $h_{u}^{l}$ and $h_{v}^{l}$. Note, the representations at $l{=}0$ are simply the node features in the original graph $\mathbf{x}_{u}$ and $\mathbf{x}_{v}$. Since we are considering the task of node-classification, there is no relation-specific representation with respect to each edge. 
% % Further, as before, we use ``sp'' which is the differentiable approximation of ReLU activation.
% For explaining node $u$'s prediction, GraphMASK generates $z^{l}_{u, v}$ for all its incident edges. Finally, the parameters $\pi$ of the erasure function are trained on multiple datapoints, and then used for explaining predictions \cite{schlichtkrull2020interpreting}. 
% % \xhdr{Lemma 1} \textit{A normalization function \text{LN} for layer $l$ is Lipschitz continuous if:}
% % \begin{equation}
% %     ||\text{LN}^{l}(\mathbf{h}_{u'}^{l}) - \text{LN}^{l}(\mathbf{h}_{u}^{l})||_{2} \leq C_{\text{LN}}^{l}~||(\mathbf{h}_{u'}^{l}-\mathbf{h}_{u}^{l})||_{2},
% %     \label{eq:lip_ln}
% % \end{equation}
% % where $C_{\text{LN}}^{l}$ is the Lipschitz constant of the normalization function for layer $l$.
% % \textit{Proof.~} The layer normalization function is a reparametrization trick that significantly reduces the problem of coordinating updates across different layers.
% % A given representation $\mathbf{h}_{u}^{l}$ is normalized using mean and standard deviation parameters that are learned during the training stage, \ie
% % \begin{equation}
% %     \text{LN}^{l}(\mathbf{h}_{u}^{l}) = \frac{(\mathbf{h}_{u}^{l}-\mu^{l})}{\varsigma^{l}},
% %     \label{eq:layer_norm}
% % \end{equation}
% % where $\mu^{l}$ is the mean and $\varsigma^{l}$ is the standard deviation of the representations at layer $l$, and are fixed after the training completes. Using Eqn.~\ref{eq:layer_norm}, the difference between the layer normalized output at layer $l$ of a perturbed and original representation can be given as:
% % \begin{align*}
% %     & \text{LN}^{l}(\mathbf{h}_{u'}^{l}) - \text{LN}^{l}(\mathbf{h}_{u}^{l}) = \frac{(\mathbf{h}_{u'}^{l}-\mu^{l})}{\varsigma^{l}} - \frac{(\mathbf{h}_{u}^{l}-\mu^{l})}{\varsigma^{l}} \\
% %     & \text{LN}^{l}(\mathbf{h}_{u'}^{l}) - \text{LN}^{l}(\mathbf{h}_{u}^{l}) = \frac{(\mathbf{h}_{u'}^{l}-\mathbf{h}_{u}^{l})}{\varsigma^{l}}
% % \end{align*}
% % Taking $L_{2}$-norm on both sides and applying Cauchy-Schwartz inequality, we get:
% % \begin{align*}
% %     & ||\text{LN}^{l}(\mathbf{h}_{u'}^{l}) - \text{LN}^{l}(\mathbf{h}_{u}^{l})||_{2} \leq ||\frac{1}{\varsigma^{l}}||_{2}~||(\mathbf{h}_{u'}^{l}-\mathbf{h}_{u}^{l})||_{2}
% % \end{align*}
% % For consistency, we define $C_{\text{LN}}^{l}{=}||\frac{1}{\varsigma^{l}}||_{2}$ as the Lipschitz constant for the $l^{\text{th}}$ normalization layer.


% \xhdr{Theorem 7 (GraphMASK Instability)} \textit{Given the concatenated representation of the original and perturbed graph, the scalar location explanation for an edge in layer $l$ is stable if:}
% \begin{equation}
%     ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq \gamma_{4}^{l}~||q^{l}_{u',v} - q^{l}_{u,v}||_{2},
%     \label{eq:gmask_stable}
% \end{equation}
% where $\gamma_{4}^{l}$ denotes the Lipschitz constant which is a product of the weights of the $l$-th fully-connected layer, and the Lipschitz constants for the layer normalization function and softplus activation function.

% \textit{Proof Sketch.~} We prove that the scalar explanation  generated by GraphMASK for an edge in layer $l$ is Lipschitz and the Lipschitz constant ($\gamma_{4}^{l}$) is product of the Lipschitz constants of the layer normalization function and the $l_{2}$-norm of the weight matrices of the erasure function.
% See Sec.~\ref{app:graphmask} for more details.

% % Using Eqn.~\ref{eq:gpi}, the scalar location parameter for a perturbed node $u'$ can be written as:
% % \begin{align*}
% %     z^{l}_{u', v} = \mathbf{W}_{2}^{l}~\text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u',v}))
% % \end{align*}
% % Note, for explanation all the parameters of the fully-connected layers are fixed as they are trained initially using a set of training datapoints.
% % \begin{align*}
% %     & z^{l}_{u', v} - z^{l}_{u, v}= \mathbf{W}_{2}^{l}~\text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u',v})) - \mathbf{W}_{2}^{l}~\text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u,v})) \\
% %     & z^{l}_{u', v} - z^{l}_{u, v}= \mathbf{W}_{2}^{l}~\big(\text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u',v})) - \text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u,v}))\big) \\
% % \end{align*}
% % Taking $L_{2}$-norm on both sides and applying Cauchy-Schwartz inequality, we get:
% % \begin{align*}
% %     & ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq ||\mathbf{W}_{2}^{l}||_{2}~||\text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u',v})) - \text{sp}(\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u,v}))||_{2}\\
% %     & \leq C_{\text{SP}}||\mathbf{W}_{2}^{l}||_{2}~||\text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u',v}) - \text{LN}^{l}(\mathbf{W}_{1}^{l}q^{l}_{u,v})||_{2}, \tag{Using Corollary 1}
% % \end{align*}
% % where $C_{\text{SP}}$ is the Lipschitz constant for the softplus activation function. Simplifying further we get:
% % \begin{align*}
% %     & ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq C_{\text{SP}}~C_{\text{LN}}^{l}||\mathbf{W}_{2}^{l}||_{2}~||\mathbf{W}_{1}^{l}q^{l}_{u',v} - \mathbf{W}_{1}^{l}q^{l}_{u,v}||_{2} \tag{Using Lemma 1}\\
% %     & \leq C_{\text{SP}}~C_{\text{LN}}^{l}||\mathbf{W}_{2}^{l}||_{2}~||\mathbf{W}_{1}^{l}||_{2}~||q^{l}_{u',v} - q^{l}_{u,v}||_{2} \tag{Using Cauchy-Schwartz inequality}
% % \end{align*}

% % Hence, for a given layer $l$ the difference between the scalar location parameter of a perturbed and original node $u$ is given by:
% % \begin{equation}
% %     ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq \gamma_{4}^{l}~||q^{l}_{u',v} - q^{l}_{u,v}||_{2},
% %     \label{eq:gmask_stability}
% % \end{equation}
% % where $\gamma_{4}^{l}=C_{\text{SP}}~C_{\text{LN}}^{l}||\mathbf{W}_{2}^{l}||_{2}~||\mathbf{W}_{1}^{l}||_{2}$. Now, for explaining the prediction for node $u$, we can repeat this process for all edges $(u,v) \in \mathcal{E}$ in the neighborhood $\mathcal{N}_{u}$ of node $u$ and generate the matrix $\mathbf{Z}^{l}$. It is to be noted, that the values of the $z^{l}_{u, v}$ elements represent whether a given edge can be dropped or not---an explanation.
% % Further, the composition of multiple Lipschitz continuous functions with Lipschitz constants $\{\mathcal{L}_1, \dots, \mathcal{L}_{\text{L}}\}$ is a new Lipschitz continuous function with $\mathcal{L}_1 \times \dots \times \mathcal{L}_{\text{L}}$ as the Lipschitz constant \cite{gouk2021regularisation}. Using the formulation for a single layer $l$ (Eqn.~\ref{eq:gmask_stability}), we can generate a bound for all $L$ layers of the model $f$, where the Lipschitz constant will be: $\prod_{l=1}^{L}\gamma_{4}^{l}$.

% \xhdr{Theorem 8 (GraphMASK Counterfactual Unfairness)} \textit{Given the concatenated representation of the original and perturbed graph, the scalar location explanation for an edge in layer $l$ is counterfactually fair if:}
% \begin{equation}
%     ||z^{l}_{u', v} - z^{l}_{u, v}||_{2} \leq \gamma_{4}^{l}~||q^{l}_{u^{s},v} - q^{l}_{u,v}||_{2},
%     \label{eq:gmask_counter}
% \end{equation}
% where $\gamma_{4}^{l}$ is the same constant as defined in Theorem 7.

% \textit{Proof Sketch.~} A counterfactual node $u^{s}$ is generated by flipping/modifying one sensitive attribute from the original node features. The left term in Eqn.~\ref{eq:gmask_counter} is similar to that of Eqn.~\ref{eq:gmask_stable} of Theorem 7. The term $q^{l}_{u^{s}}$ denotes the counterfactual representation due to node $u^{s}$. Note, for the first layer, the right term of Eqn.~\ref{eq:gmask_counter} simplifies to just $\gamma_{4}^{l}$ as the $p$-norm between the original and counterfactual node features is one, \ie $||\mathbf{x}_{u^{s}}-\mathbf{x}_{u}||_{p}{=}1$.
% , as all their individual node features are the same except the sensitive attribute which is flipped.

==> 080ethics.tex <==
While several classes of GNN \expmethods have been proposed in recent literature, there is little to no understanding as to which of these approaches are more effective than the others and/or if some of these approaches are better suited for certain kinds of real-world applications.
This lack of understanding not only limits the applicability of GNN \expmethods in practice but also hinders the progress of research in graph XAI. To this end, decision-makers can use our theoretical framework to analyze GNN \expmethods for understanding the robustness and biases in GNN models before deploying them in real-world applications. Stakeholders in real-world settings may use our analysis to determine which \expmethods to employ. 

==> 090reproducibility.tex <==
\looseness=-1
We introduce the first-ever theoretical analysis of state-of-the-art GNN explanation methods (Section~\ref{sec:properties}). We explain and detail all the assumptions and complete proofs (Appendix~\ref{app:sec_proof}) for establishing the upper bounds on the violation of faithfulness, stability, and fairness properties. In addition, a link to an anonymous downloadable source code is included as part of the supplementary materials, along with a readme file of how to reproduce the main experimental results. We provide a brief overview of the training and implementation details (Sec.~\ref{sec:exp}) and a detailed description of our experimental setup in Appendix~\ref{app:sec_experiment}. We include the total amount of compute and the type of resources used in Appendix~\ref{app:sec_experiment}.
